GLAD: Group Anomaly Detection in Social Media Analysis- Extended Abstract

Traditional anomaly detection on social media mostly focuses on individual point anomalies while anomalous phenomena usually occur in groups. Therefore it is valuable to study the collective behavior of individuals and detect group anomalies. Existing group anomaly detection approaches rely on the assumption that the groups are known, which can hardly be true in real world social media applications. In this paper, we take a generative approach by proposing a hierarchical Bayes model: Group Latent Anomaly Detection (GLAD) model. GLAD takes both pair-wise and point-wise data as input, automatically infers the groups and detects group anomalies simultaneously. To account for the dynamic properties of the social media data, we further generalize GLAD to its dynamic extension d-GLAD. We conduct extensive experiments to evaluate our models on both synthetic and real world datasets. The empirical results demonstrate that our approach is effective and robust in discovering latent groups and detecting group anomalies.

==> discussion.tex <==
% discussion
\xhedit{As we provide a systematic approach for group anomaly detection in this work, our study does have certain limitations.}
\xhedit{Though the} particular type of group anomaly \xhedit{discussed} in this paper has found applications in astronomy \cite{xiong_hierarchical_2011}, particle physics \cite{muandet_one-class_2013} and fluid mechanics \cite{xiong_group_2011}. However, \xhedit{we still face} the challenges of obtaining ground truth labels \xhedit{for} performance evaluation \xhedit{when detecting group anomalies in social networks}. \xhedit{In this work, we mainly} resort to anomaly injection to showcase the power of our model. For real world applications, \xhedit{with no ground truth anomaly labels and lack of knowledge in the types of possible anomalies, we limit ourselves to examination of the modeling power of our generative models and providing anecdotal explanations.}
%as we do not know the definition of group anomaly beforehand, we can hardly conduct anomaly injection. 


\xhedit{In addition, we assume that both the number of groups and the number of roles are given as input to the inference and learning algorithms. As a result, for the experiments on senator and publication datasets, we manually pick the model hyper-parameters based on our prior knowledge of the data. Though we do not fully address the problem of model selection for our analysis, non-parametric models could be incorporated to achieve a graceful solution of this problem as a future work.}

in this work, we do not fully address the problem of model selection for our analysis. For the experiments on senator and publication datasets, we pick the model hyper-parameters based on our prior knowledge of the data. Non-parametric models could be a more graceful solution to this problem. Finally, the computational complexity of GLAD with variational inference is linear to the sample size. But for d-GLAD, given the complexity of the model and the particle filtering approach, it is not very well scalable. As a follow-up work, applying variational method for d-GLAD or paralleling the sampling procedure could achieve further speed-up.


==> simulation.tex <==
% Simulation
To compare the anomaly detection performance of the proposed alternative model, we conducted a simulation with injected group anomalies. We generate a network with 500 individuals using GLAD in Algorithm \ref{alg:genGLAD}. To evaluate the anomaly detection performance, we set the mixture rates of anomalous groups as $[0.9, 0.1]$ and normal groups as $[0.1,0.9]$. We vary the number of groups from 5 to 50 and inject $20\%$ anomalous groups. The rest $80\%$ groups are normal. Since we know the normal and anomalous mixture rates, we calculate the anomaly score of each group by directly computing the differences between the inferred mixture rate and the ground truth normal mixture rate. During the testing procedure, we rank the groups with respect to their anomaly score and retrieve top $20\%$ groups.  For all methods, we set the number of groups and number of roles the same as the ground truth. .

We compare the alternative GLAD model ( GLAD in the plot) with the following four baselines.
\begin{enumerate}
\item\textbf{MMSB-LDA}:First use the MMSB model to learn a group membership distribution for each individual node, then assign the node to the group with the highest probability. Finally, for each group, train an LDA model and infer the role identity.
\item \textbf{MMSB-MGM}: Group is learned using the same method as MMSB-LDA. For the role inference,  train an multi-modal MGM instead of LDA.
\item \textbf{Graph-LDA}: Run an off-the-shelf graph clustering algorithm Min-Cut to get group membership and then train a LDA model for each group.
\item \textbf{Graph-MGM}: Get group membership with the graph clustering algorithm Min-Cut and then train a MGM model for each group.
\end{enumerate}
\begin{figure}[t]
\centering
\includegraphics[scale = 0.46]{./fig/synthetic_errorbar_glad2.pdf}
\caption{ Detection accuracy error bar plot of the alternative GLAD model and baseline methods on synthetic dataset of 500 samples with respect to group number from 2 to 10, with $20\%$ anomalous groups.}
\label{fig:syn_anomaly}
\end{figure}
Figure \ref{fig:syn_anomaly} shows the anomaly detection performance comparison with number of groups varying from 1 to 10  for the alternative GLAD model and four other baselines. For most of the cases (expect for group number 8 and 9), the alternative GLAD model achieves the highest detection accuracy, while the other two-stage approaches are relatively unstable.  The performance deterioration of the proposed model is due to the sparsity of the data. As we increase the number of groups for a fix size network, each group has fewer number of people, thus learning the role mixture for the group becomes more difficult.
